The International Linear Collider: Report to Snowmass 2021

The International Linear Collider (ILC) is on the table now as a new global energy-frontier accelerator laboratory taking data in the 2030s. The ILC addresses key questions for our current understanding of particle physics. It is based on a proven accelerator technology. Its experiments will challenge the Standard Model of particle physics and will provide a new window to look beyond it. This document brings the story of the ILC up to date, emphasizing its strong physics motivation, its readiness for construction, and the opportunity it presents to the US and the global particle physics community.

==> chapters/gen-phys/figures/gen-phys.tex <==


[5 pages; corresponding editors: Daniel Jeans (daniel.jeans@kek.jp),
Jenny List (jenny.list@desy.de), Michael Peskin (mpeskin@slac.stanford.edu)]


This  chapter gives a general orientation to the physics of the ILC.  We will describe the major physics processes that the ILC will allow us to study, and reactions that appear as backgrounds in the analyses discussed in Chapters 8--10.  

We will also call attention to the effects of beam polarization.  Beam polarization is not an important parameter for proton-proton collisions, first, because it is difficult to prepare highly polarized proton beams and, second, because the spin of a proton is divided among the quarks and gluons in a complex way.   For electrons, the story is different.   Because the electron is an elementary particle, its polarization is transferred directly into any reaction. Longitudinal polarization is maintained in linear acceleration, so that a highly polarized source of electrons or positrons produces a comparable effect of polarization in collisions.  Further, in the SM, highly relativistic left- and right-handed polarized electrons are essentially different species, with different electroweak quantum numbers.  Thus, measurements with different beam polarization measure different reactions, and the comparison of these reaction rates can give direct insight into the physics.

%Figure 1
%%%%%%%%%%%%%%%%
\begin{figure}
 \begin{center}
\includegraphics[width=0.80\hsize]{chapters/gen-phys/figures/crosssections.pdf}
\end{center}
\caption{Cross sections of the most important Standard Model processes in $\ee$ annihilation in the energy range of the ILC.  Initial state radiation is included, and cross section are plotted for reactions in which the annihilation retains $>90\%$ of the nominal CM energy.  For simplicity, the cross sections are computed with zero beam polarization and ignoring beamstrahlung.}
\label{fig:crosssections}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\section{Key Standard Model Processes}
\label{sec:SMprocesses}

The major reactions at $\ee$ colliders in the energy range of 100~GeV to 1~TeV are shown in Fig.~ref{fig:crosssections}.   The typical size of a cross section in $\ee$ annihilation is the point
cross section
\beq
          1~\mbox{R} =   {4\pi \alpha^2\over 3E_{CM}^2} =  1.4 ~\mbox{pb} \cdot \biggl( {250~\mbox{GeV} \over E_{CM} } \biggr)^2 \ ,
\eeqn
corresponding to several million events in a data set of 2~ab$^{-1}$ at 250~\mbox{GeV}.   This is a much smaller number of events than is typically collected by a hadron collider experiment.  However,
these events appear individually in $\ee$ bunch collisions, are essentially free of extra tracks and debris associated with the beams, and are reconstructable with high efficiency over an angular region that extends to within milliradians of the beam directions.  The simplicity of typical events allows the use of detector technologies with high degrees of discrimination and precision, as will be discussed in the next chapter.

Since the electron is an elementary particle, the basic parameters of the ILC beams are very well understood.   Though the beams contain a distribution of electron and positron energies due to 
initial state photon radiation and radiation of photons in the beam-beam interaction (``beamstrahlung''), these are minor and computable effects.   There is no analogue of the nonperturbative parton distributions needed for the interpretation of cross sections at hadron colliders.  Similarly, the beam polarizations can be measured both by dedicated detectors and through SM processes with large cross sections.    Thus, the ILC can carry out precision measurements of absolute cross sections in addition to asymmetries and distributions.

Each of the reactions shown in the figure has its own individual role in the program of the ILC.  Each reaction gives access to its own set of precision tests of the Standard Model and searches for the effects of new physics.   It is also important to understand the hierarchy of reactions to understand the important sources of background that enter the various analyses.  At an $\ee$ collider, backgrounds from simple QED and QCD processes are readily eliminated.   The major backgrounds to processes with the production of heavy particles---within the SM, $W$, $Z$, Higgs, and top---are other reactions with heavy SM particles in the final state.

The simplest reaction in $\ee$ annihilation is that of $\ee\to f\bar f$, where $f$ can be a quark or a lepton.   Even for the hadronic reactions, the final state is typically two narrow jets and is easily discriminated from reactions of electroweak bosons.   At the tree level in the SM, the differential cross section is very simple.  For example, for 100\% left-handed polarized beams and $s \gg m_Z^2$, the differential cross sections are  
\beq
  {  d\sigma\over d\cos\theta} =  {\pi \alpha^2\over 2s} \bigg[ (\half I^3_{fL}  + \half Y_{fL})^2) (1 + \cos\theta)^2 + (\half Y_{fR})^2 (1 - \cos\theta)^2 \biggr] \ ,
\eeq{FBQnos}
where $(I^3_{fL}, Y_{fL})$ are the electroweak quantum numbers of $f_L$ and $(0, Y_{fR})$ are the 
electroweak quantum numbers of $f_R$.   Note the the production of the two helicity states of $f$ separates into the two hemispheres. Thus, with two  different values for the beam polarization and separate measurment of the forward and backward cross sections, it is possible to probe all four 
individual helicity states in this reaction.  This provides a powerful and specific probe for new physics, as we will discuss in Sec.~\ref{sec:pairs500}.  Bhabha scattering ($\ee\to \ee$) has a more complex differential cross section, but this reaction is extremely well understood within the SM, leading to its own set of new physics tests.

The reaction $\ee\to$ hadrons is also an exceptionally clean setting for studies of jets and the measurement of fragmentation functions.  The potential ILC contributions to QCD, including new observables sensitive to jet substructure, are described in Sec.~\ref{sec:QCD}.

The annihilation reaction with the largest cross section in this energy region is $\ee\to W^+W^-$.   This reaction is forward-peaked, due to the contribution from a diagram with $t$-channel neutrino exchange.   The reaction can be reconstructed in all $W$ decay modes, with the most complex final states having 4 jets.  This reaction obtains contributions from diagrams with the triple gauge couplings $WW\gamma$ and $WWZ$.  Because of a cancellation among the SM diagrams required by the unitarity of that theory, the angular distributions and polarization effects in this reaction are exceptionally sensitive to  new physics contributions to the triple gauge couplings.   These effects are most pronounced in the central and backward $W^+W^-$ production. We will discuss the measurement of 
these effects in Sec.~\ref{sec:Wboson250} and Sec.~\ref{sec:Wboson500}.   In contrast, the forward production is essentially  model-independent. Because the neutrino exchange diagram requires left-handed electrons and right-handed positrons, the forward production has a large polarization asymmetry and so provides a very useful {\it in situ} measurement of beam polarization.

The other vector boson pair production reactions, $\ee\to \gamma\gamma, Z\gamma, ZZ$, do not involve triple gauge couplings in the Standard Model.   It can be shown that the new physics corrections to these reactions are also suppressed in the description of new physics by Effective Field Theory. Thus, these reactions can provide fundamental test of the Effective Field Theory framework, and, in some cases, tests of general  positivity theorems of Quantum Field Theory.  We will discuss these 
issues in Sec.~\ref{sec:generalEFT}.

The reaction $\ee\to \gamma Z$ with $\gamma$s almost collinear to the beam direction provides a large source of $Z$ bosons that can be used to probe the $Z$ properties even at CM energies well above the $Z$ resonance. In the ILC run at 250~GeV, we expect to study about 90 million $Z$ bosons in this ``radiative return'' reaction, leading to an improvement of a factor of 10  in the precision of $\sstw$ even without running at the $Z$ resonance.   The study of this reaction will be discussed in 
Sec.~\ref{sec:radreturn}.

At 250~GeV, the dominant reaction for production of the Higgs boson is $\ee\to ZH$.    This process is expected to produce about half a million Higgs bosons in the 250~GeV run of the ILC, with each Higgs boson tagged by a recoiling $Z$ boson.   This will give an excellent setting for the  measurement of SM and non-Standard Higgs boson decays.  That study will be described in Secs.~\ref{sec:Higgs250} and 
\ref{sec:HiggsExotic}.

The ILC also expects a number of reactions with photons in the initial state.   The photons arise as virtual photons from initial-state radiation and as real photons emitted in the beam-beam 
interaction (``beamstrahlung'').   For the ILC accelerator parameter sets, these two sources contribute roughly equally to the spectrum of initial photons.   Important reactions due to initial-state photons are single $W$ production ($e  \gamma \to W \nu$) and single $Z$ production ($e \gamma \to Z e$).
Reactions with two photons in the initial state include photon annihilation to lepton pairs, quark pairs, and $W^+W^-$.   The single boson production reactions have a role in the precision determination of 
the $W$ and $Z$ masses, as will be described in Sec.~\ref{sec:WZmasses}.  All of these processes appear as the major backgrounds to new particle searches involving missing energy, as discussed 
particularly in Secs.~\ref{sec:newparticles} and \ref{sec:Dark500}.

The cross sections for $\gamma\gamma$ production at large angle decrease as $1/s(\gamma\gamma)$.   The converse of this statement is that there is a large cross section for 
$\gamma\gamma$ annihilation to quarks and leptons at the lowest possible CM energies.   This leads to an ``underlying event'' giving  a few tracks in each $\ee$ bunch crossing.  We  find that this 
background has a negligible effect on our analyses.

At energies  above 250~GeV, the initial electrons and positrons can radiate $W$ and $Z$ bosons and these can interact to produce SM and, possibly, new particles by vector boson fusion.   The cross sections for these processes   rise as  $\log(s/m_W^2)$ and so above 500~GeV they become the dominate modes of heavy particle 
production.   The coupling of the  electron to the $Z$ is rather small, so the ratio of the $ZZ$ to $WW$ luminosities is 
\beq
       \biggl[ { (\half - \sstw)^2 + (\sstw)^2)\over \cstw} / {\half} \biggr]^2  =  1\%
\eeqn
for unpolarized beams, and even smaller for polarized beams enhanced in the  $e^-_Le^+_R$ initial state.  Thus, $WW$ fusion plays the dominant role.   The most important processes here are $WW$ fusion to a single $Z$ ($\ee\to \nu\bar\nu Z$) and to a single Higgs boson (($\ee\to \nu\bar\nu H$).

The process $\ee\to \nu\bar\nu H$ begins to dominate the $\ee\to ZH$ process at about 400~GeV.
Above this energy, the $WW$ fusion process provides a second, independent data set for the study of Higgs boson couplings. In the $WW$ fusion events, the Higgs boson appears as a heavy, centrally-produced particle with no other visible activity in the event.  The fact that the Higgs boson can be produced in two distinct ways at $\ee$ colliders allows cross-checks of any anomalies with the same experimental program.   This is another of the special benefits of studying the Higgs boson through $\ee$ annihilation.   The study of the Higgs boson in $WW$ fusion will be discussed in detail in Sec.~\ref{sec:HiggsWW}.

The threshold for top quark pair production $\ee\to t\bar t$, occurs in the region around of CM energy of 340--345~GeV.    At and above this energy, the ILC can study the couplings of the top quark with a high precision.  Of special interest are the electroweak couplings of the top quark, which have secondary importance at hadron colliders but provide the primary pair production mechanism at 
$\ee$ colliders.   These couplings can be especially sensitive to new physics corrections, especially in models in which the Higgs boson is composite.   Also, because the top quark theshold is a very narrow feature, the measurement of the threshold shape can give a very direct and accurate measurement of the top quark mass.  We will discuss all of these issues in Sec.~\ref{sec:top}.

At the highest ILC energies, it is also possible to access multi-boson production processes.  The most important of these are the reactions $\ee\to Z H H $ and $\ee\to \nu\bar\nu HH$, which depend
directly on the Higgs boson self-coupling, and $\ee\to t\bar t H$, which directly measures the Higgs boson coupling to the top quark.   We will discuss these analyses in Sec.~\ref{sec:Higgs500}.

Thus, each separate ILC reaction has a role to play in challenging the predictions of the SM.  But, even 
further, we do not need to interpret the individual processes in isolation from one another.  By 
interpreting the SM and its possible corrections in Effective Field Theory, the contributions from the 
different reactions can be brought together and applied in a unified way.    The whole set of ILC 
measurements is then more powerful than the simple sum of its parts.   We will discuss this 
strategy of interpretating the ILC measurements in some detail in Chapter 12.



%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.90\hsize]{chapters/gen-phys/figures/lumi_H20-staged.pdf}
\end{center}
\caption{Plan for the operation of the ILC through its various stages from 250~GeV to 500~GeV.
The details of this program most relevant for physics studies are shown in Table~\ref{tab:staging-phys}.   The detailed accelerator parameters for each stage are given in 
Table~\ref{tab:ilc-params}.   The total length of the program is 22~years.   Additional stages at the $Z$ boson resonance and at 1~TeV could be added to this plan.   Parameters for these programs are also 
presented in the tables.}
\label{fig:ILC-staging}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Energy and Luminosity}
\label{sec:EvsL}

As we have discussed already in Sec.~\ref{sec:acc-staging}, the ILC is designed to be upgraded, in stages, in energy and luminosity.  Our current plan for the energy and luminosity evolution of the ILC is shown in Fig.~\ref{fig:ILC-staging}.    The parameters of the successive stages that are most important for understanding the physics studies are shown in Table~\ref{tab:ILC-staging}.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{center}
\begin{tabular}{lccccc}
                                     &  91 GeV &     250 GeV  &   350 GeV   &   500 GeV &   1000 GeV \\ \hline
$\int  \L$ (ab$^{-1}$)     &      0.1      &    2           &        0.2       &     4         &      8    \\     
duration (yr)                  &        1.5         &       11          &    0.75                &     9           &      10      \\ 
beam polarization ($e^-/e^+$; \%)   &   80/30  &  80/30    &  80/30  &   80/30  &  80/20  \\
(LL, LR, RL, RR)  (\%)          &  (10,40,40,10) & (5,45,45,5) &  (5,68,22,5) &  (10,40,40,10) 
               & (10,40,40,10) \\
$\delta_{ISR}$ (\%)       &    10.8      &    11.7              &         12.0               &      12.4             &                13.0                \\ 
$\delta_{BS}$  (\%)       &       &   2.6            &                        &       4.5            &      10.5          
\end{tabular}
\end{center}
\caption{Parameters of the successive ILC stages most relevant for physics studies. The value given here are those 
actually used for the results to be quoted in this report.   The fourth line 
gives the fraction of the total running time spent in each of the four possible beam polarization 
orientations.  The fifth and sixth lines give the average energy loss to initial state radiation
and beamstrahlung, respectively.}
\label{tab:ILC-staging}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

The last lines of the table show the average fractional energy loss to initial state radiation and 
beamstrahlung.    The $e^+e^-$, $e\gamma$, and $\gamma\gamma$ luminosity spectra for the various stages are shown in Fig.~\ref{fig:eglumis}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
%\begin{center}
% \includegraphics[width=0.90\hsize]{chapters/gen-phys/figures/eglumis.pdf}
% \end{center}
\caption{Luminosity spectra for $e^+e^-$, $e\gamma$, and $\gamma\gamma$ annihilation 
reactions for each of the designs in Table~\ref{tab:ILC-staging}.    The $x$ axis in each graph is the effective 
CM energy as a fraction of the nominal CM energy.}
\label{fig:eglumis}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


Our plan for the ILC begins with collisions at 250~GeV and a 
modest luminosity of  $1.35\times 10^{34}$ cm$^{-2}$sec$^{-1}$.    This luminosity would then be 
doubled by doubling the number of accelerated bunches per RF pulse, an upgrade that only requires the addition of RF power.  
in about 11 years, the ILC will have accumulated a total integrated luminosity of  2~ab$^{-1}$.
This will be followed by an energy upgrade, which entails lengthening the linear accelerators to double their energy.   The 
parameters in the table assume the current ILC accelerator parameters for this upgrade, but this 
will be less costly if higher-gradient superconducting RF cavities are available at that time.   The 
500~GeV stage will accumulate 4~ab$^{-1}$ of integrated luminosity at 500~GeV, with also 200~fb$^{-1}$ of luminosity near 350~GeV to measure the top quark mass to the level of
the theoretical systematic errors.

Two additional runs could be added to this plan.  The first is a run at the $Z$ boson resonance, accumulating about $5\times 10^9$ $Z$ bosons.   The accelerator parameters 
for this ``Giga-Z'' program have been discussed in Sec.~[need this section in the acc. chapter].
If this run is done after the installation of RF for the 250~GeV luminosity upgrade, the $Z$ program would take about 2 years.    The second is a run at 1~TeV, requiring a second lengthening of the 
linear accelerator.  Since the luminosity of a linear collider naturally increases roughly linearly with 
the center  of mass energy, we expect that the 1~TeV operator will accumulate 8~ab$^{-1}$ if
integrated luminosity in a 10-year program.

All of this data-taking will benefit from the expected high degree of polarization of the electron beam and the planned polarization of the positron beam.    At  1~TeV, where the main object of study will be the $WW$ fusion reactions, this benefit can be enhanced by chosing to operate predominantly with 
$e^-_Le^+_R$-polarized beams.

This plan for the evolution of the ILC is based on a detailed optimization study based on the physics 
goals, carried out in 2015~\cite{Barklow:2015tja}.   Of course, the plan is can be revised according to new developments in particle physics and superconducting RF technology. 
 

\section{Beam Polarization}
\label{sec:polarization}

The ILC design includes beam polarization for both electron and positrons.   This allows the polarization to be used in experiments in a number of different ways.   In this section, we will summarize these and provide the polarization measures appropriate to each case.   More details can be found
in the individual analysis described below.

The ILC design calls for electron polarization of 80\% and positron polarization of 30\%.  Both signs of the polarization will be available in each run.  It is important that the polarization be flipped as often as possible to cancel systematic errors from drifts of detector parameters.   For both beams, the polarization can be flipped pseudo-randomly bunch train by bunch train.  For the electron beam, this is done at the sourcer by controlling the polarization of the laser used to stimulate electron emission from the cathode. This is similar to the scheme used in the SLD experiment~\cite{Woods:1996ph}.  For the positron beam, the 
polarization is flipped by spin rotators appropriately placed  downstream of the helical undulator~\cite{Malysheva:2016jdr}.

The polarization of a beam containing $N_L$ left- and $N_R$ right-handed particles is given by 
\beq
                 P =    {N_L - N_R\over N_L + N_R}
\eeqn
Since typically cross sections for left-handed electrons are larger, we will take left-handed polarizations to give positive $P$ in this discussion.
Then a beam of polarization $P$ contains the fractions of particles of each helicity
\beq
             f_L = {1 + P\over 2}           \qquad     f_L = {1 -  P\over 2}
\eeqn
For the ILC polarizations, the   $e^-_L$ and  $e^+_L$ beams have the content
\beq
         f_R(e^-_L) =   90\%         \qquad   f_L(e^-_L) = 10\%  \qquad   f_R(e^+_L) =  65\%  qquad     f_L(e^+_L) = 35\%  
\eeqn
Since the $e^-_R$ and $e^-_L$ have different $SU(2)\times U(1)$ quantum numbers, each of the four polarization settings is effectively a different 
scattering experiment.   The results of the four experiments can be combined in various ways for different purposes.   We describe four of these 
here.

{\bf Cross section asymmetries:}
Because of helicity conservation in vector boson couplings, $\ee$ annihilation reactions proceed only from the $e^-_Le^+_R$ and $e^-_Re^+_L$ helicity 
combinations.   Typically, in annihilation to fermions, these two cross sections differ by a factor of 2.  (Specifically for $\ee\to ZH$, the cross sections 
differ by a factor 1.4.).   If we write the two cross sections for 100\% polarized initial states as
\beq
        \sigma = \sigma_0 (1 \pm   {\cal A} )
\eeqn
with $+$ for pure $e^-_Le^+_R$ and $-$ for pure $e^-_Re^+_L$
Then the cross section for electron and positron polarizations  $P_{e}$ and $P_{p}$ is
\beqa
            \sigma(P_e, P_p) =    f_L(e) f_R(p)  \sigma_0 (1 +{\cal A} ) +  f_L(e) f_R(p)  \sigma_0 (1 -  {\cal A} )  \CR
                                      &=&   \biggl({ 1  - P_eP_p  \over 2}\biggr) \sigma_0  + \biggl({P_e - P_p\over 2}) \sigma_0 {\cal A}
\eeq{CSpol}
The asymmetry $A$ between the cross sections with $LR$ and $RL$ polarized beams is then
\beq
                          A  =    P_{eff}  {\cal A}   \qquad   \mbox{with} \qquad    P_{eff} =  { P_e - P_p \over  1  - P_eP_p  }   =  89\% \ ,
\eeq{CSasym}
for 80\%/30\%  beam polarizations at the ILC.   For this measurement of the intrinsic polarization asymmetry, many sources of systematic error cancel out, including the absolute luminosity and the absolute detector acceptance.   It is necessary that the beam intensities be the same for left- and right- handed
beams, which is insured if the polarization is flipped rapidly, and that the detector acceptance be very accurately forward-backward symmetric.   The measurment of ${\cal A}$ does depend strongly on the absolute knowledge of the polarization.  At the ILC, we plan to use multiple methods to bring the systematic error on the polarization down to $5\times 10^{-4}$. [ ref to where this is described in the report ] 

It is clear already from eq.~\leqn{FBQnos} that the polarization asymmetric ${\cal A}$ gives direct information on the quantum numbers of the particles participating in an $\ee$ annihilation reaction. As we will see in Sec.~\ref{sec:expectations}, the polarization asymmetry in the reaction $\ee\to ZH$ also plays an outsize role in the global analysis using Effective Field Theory that determines the Higgs boson couplings.  It is then remarkable that this quantity can be obtained so precisely using polarized beams.

{\bf Cross section enhancements:}
Another results of eq. \leqn{CSpol} is that, if the physics of a process very much favors the $e^-_Le^+_R$ helicity state, beam polarization gives an 
enhancement of the effective luminosity.   For $WW$ fusion reactions, which appear only from the  $e^-_Le^+_R$ initial state, the effective luminosity
for $e^-(L)e^+(R)$ polarized beams is enhanced from that for unpolarized beams by the factor
\beq  
    {\cal L}_{eff}/{\cal L}   =  (1 + P_e)(1-P_p)  =   2.3
\eeq{lumienhance}
for 80\%/30\%  beam polarizations at the ILC.

In practice, one should not try to achieve the full promised luminosity enhancement.  Each physics process has its own dependence on polarization, and it is also important to reserve some of the luminosity for data on the modes with smaller  production cross sections.  This is reflected in our choice of the 
division of polarization modes in line 4 of Table~\ref{tab:ILC-staging}.   The run at the top quark threshold has a quite specific goal, and running with mainly $e^-(L)e^+(R)$ polarized beams is optimal for this.  At other energies, where the physics program is more general, the fraction of polarizations used should be optimized taking into account the uses in the next two sections.

{\bf Background reduction:}
Especially for reactions that include neutrinos or other sources of missing energy, the process $\ee \to W^+W^-$ is a the dominant source of background.   It is therefore important that the cross section for $\ee\to W^+W^-$ is dramatically reduced in the $e^-_Re^+_L$ initial state. Backgrounds from photon-induced processes such as $\gamma\gamma\to \ell^+\ell^-$  and single $W$ production are still present in the $e^-_Le^+_L$ and 
$e^-_Re^+_R$ samples, while the annihilation reactions cannot appear.   This ability to reduce some relevant backgrounds and to directly measure others can be crucial in measuring the rates of these processes precisely or, in the case of particle searches, establishing strong limits.

This is illustrated for a search for dark matter pair production that will be described in Sec.~\ref{sec:newparticles}.   Fig.~\ref{fig:DMpol} shows the results of a simulated search for dark matter pair production $\ee\to \chi\chi$  at
 500~GeV~\cite{Habermehl:2018yul}.  The analysis assumes no signal and puts a lower limit on an Effective Field Theory parameter.  What concerns us now
 is the left-hand plot,  which  includes statistical errors only.   The red (short-dash) curve shows the limit from the 
mixture of polarization states in Table~\ref{tab:ILC-staging}.  The figure shows 
 that almost all of the exclusion comes from the 40\% of the run that is collected with the $e^-(R)e^+(L)$ beam configuration.
However, there is a second half to this story, which is explained below.

%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.42\hsize]{chapters/gen-phys/figures/vector_noSystematics.pdf}\ \ 
\includegraphics[width=0.42\hsize]{chapters/gen-phys/figures/vector_withSystematics.pdf}
\end{center}
\caption{Limits on an Effective Field Theory mass scale associated with dark matter particle pair production in $\ee$ annihilation from a search simulation at 500~GeV, showing the dependence of the results on beam polarization, from \cite{Habermehl:2018yul}.  Higher limits are better.   In both figures, the black curve is an analysis for unpolarized beams, the red (short-dash) curve corresponds to the mixture of  polarization states  in Table~\ref{tab:ILC-staging}.    Left: analysis with 
statistical errors only; Right:  analysis including both statistical and systematic errors.}
\label{fig:DMpol}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



{\rm Control of systematic errors:}
With its four configurations for the polarization of the electron and positron beams, the ILC will be  carrying out four  different experiments simultaneously.  These four data samples have very different mixes of physics processes, with $\ee$ annihilation reactions essentially missing from the $e^-(L)e^+(L)$ and $e^-(R)e^+(R)$ samples while non-annihilation processes remain.  However, with rapid polarization flipping, the experiments will be done in the same detector.  This allows nuissance parameters associated with detector acceptance and energy response to measured by comparison the different samples.  The potential 
systematic errors associated with these parameters can thus be greatly reduced.

As an example of an application of this strategy, look now at the right-hand plot in Fig.~\ref{fig:DMpol}.   Nominally, uncertainties from knowledge of the detector would weaken the observed limits, and this effect is visible in the black curve 
giving the result for unpolarized beams and in the curves for individual polarization states.  However, the use of a  mix of 
polarization states including the nominally unproductive helicity-violating configurations, can be used to evaluate the 
uncertain detector  parameters and retain most of the power of the analysis including only statistical errors.

In processes subject to smaller systematic errrors, it is more  difficult to quantitatively express the advantage of positron polarization.   A small advantage from the enhancement of cross sections is be compensated by the loss of productive 
luminosity in measuring the samples with helicity-violating polarization configurations.  However, the use of positron polarization leads to double the number of individual data sets, adding redundancy and cross-checks.  The goal of the ILC is to 
discover that the physics of $\ee$ annihilation differs from the predictions of the Standard Model.  These check could prove 
essential in making that case.
